Safety in Augmented Importance Sampling: Performance Bounds for Robust MPPI

This work explores the nature of augmented importance sampling in safety-constrained model predictive control problems. When operating in a constrained environment, sampling based model predictive control and motion planning typically utilizes penalty functions or expensive optimization based control barrier algorithms to maintain feasibility of forward sampling. In contrast the presented algorithm utilizes discrete embedded barrier states in augmented importance sampling to apply feedback with respect to a nominal state when sampling. We will demonstrate that this approach of safety of discrete embedded barrier states in augmented importance sampling is more sample efficient by metric of collision free trajectories, is computationally feasible to perform per sample, and results in better safety performance on a cluttered navigation task with extreme un-modeled disturbances. In addition, we will utilize the theoretical properties of augmented importance sampling and safety control to derive a new bound on the free energy of the system.

==> RSS 2022: Safety in Augmented Importance Sampling: Performance Bounds for Robust MPPI/commands.tex <==
% Base tex file for reusable commands

% Vector Variables
\newcommand{\vx}[0]{\mathbf{x}}
\newcommand{\vu}[0]{\mathbf{u}}
\newcommand{\vw}[0]{\mathbf{w}}
\newcommand{\vp}[0]{\mathbf{p}}
\newcommand{\vq}[0]{\mathbf{q}}
\newcommand{\vv}[0]{\mathbf{v}}
\newcommand{\vz}[0]{\mathbf{z}}
\newcommand{\vxdot}[0]{\dot{\vx}}
\newcommand{\ve}[0]{\mathbf{e}}
\newcommand{\argmax}{\operatornamewithlimits{argmax}}
\newcommand{\argmin}{\operatornamewithlimits{argmin}}


% Transpose
\newcommand{\rT}[0]{{\textrm{T}}}

% Trajectories
\newcommand{\xtraj}[0]{\mathbf{x}_{\tau}}
\newcommand{\utraj}[0]{\mathbf{u}_{\tau}}

% Domains
\newcommand{\real}[0]{\mathbb{R}}
\newcommand{\domain}[0]{\mathcal{D}}
\newcommand{\safeset}[0]{\mathcal{C}}

% Probability Distributions
\newcommand{\Pb}[0]{\mathbb{P}}
\newcommand{\Qb}[0]{\mathbb{Q}}
\newcommand{\gaussian}[2]{\mathcal{N}(#1, #2)}

% KL Divergence
\newcommand{\KL}[2]{\mathbb{KL}\left({#1}\parallel {#2}\right)}

% Expectation
\newcommand{\ExP}[2]{\mathbb{E}_{#1}\big[ #2 \big]}

% Math
\newcommand{\pluseq}{\mathrel{+}=}


%% Acronyms
\begin{acronym}
\acro{MPPI}{Model-Predictive Path Integral Control}
\acro{Tube-MPPI}{Tube Model-Predictive Path Integral Control}
\acro{RMPPI}{Robust Model-Predictive Path Integral Control}
\acro{CCM}{Control Contraction Metrics}
\acro{MPC}{Model-Predictive Control}
\acro{IS}{Importance Sampling}
\acro{KL}{Kullback–Leibler}
\acro{GT-ARF}{Georgia Tech Autonomous Racing Facility}
\acro{iLQG}{iterative Linear Quadratic Gaussian}
\acro{AIS}{Augmented Importance Sampling}
\acro{SAIS}{Safe Augmented Importance Sampling}
\acro{CBFs}{Control Barrier Functions}
\acro{SA-RMPPI}{Safety Augmented Robust Model Predictive Path Integral Control}
\end{acronym}


==> RSS 2022: Safety in Augmented Importance Sampling: Performance Bounds for Robust MPPI/packages.tex <==
% Algorithms
\usepackage[ruled,vlined]{algorithm2e}

% References
\usepackage{cleveref}

% Acronyms
\usepackage[nolist]{acronym}

% Figures
\usepackage{subfig}

\usepackage{xcolor}

\usepackage{amsthm}
\newtheorem{condition}{Condition}
\newtheorem{lemma}{Lemma}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{definition}{Definition}[section]
\newtheorem{proposition}[theorem]{Proposition}
